A New 5 bit/2D-symbol Modulation Format for Relative Intensity Noise-dominated IM-DD Systems

We propose a novel 5-bit/2D-symbol modulation format based on PAM-6 optimized for IM-DD systems dominated by relative intensity noise. The proposed modulation scheme improves SNR by 0.94 dB compared to conventional PAM-6 and achieves near-optimal BER performance.

==> FigTikZ/MI_plot.tex <==
\definecolor{my_green}{rgb}{0.55, 0.71, 0.0}    %en la variables "my_green" guardo un color que he definido a partir de las componentes RGB. Es recomendable definir colores porque las librerías de tikZ no suelen tener mucha variedad de colores.
\definecolor{my_purple}{rgb}{0.5, 0, 0.5}
\definecolor{azure}{rgb}{0, 0.5, 0.5}

\pgfmathsetmacro{\lw}{0.6}    % lines
\pgfmathsetmacro{\lww}{0.5}    % markers

\pgfplotstableread{FigTikZ/data_txt/RIN_141_SER_MI_symbolwise.txt}\datatableSW

\newcommand{\blacksolid}{\raisebox{2pt}{\tikz{\draw[color=black,solid,line width=\lw,mark=o,mark options={solid}](0,0) -- (5mm,0);}}}   %Símbolo de curva solida
\newcommand{\blacksdashed}{\raisebox{2pt}{\tikz{\draw[color=black,dashed,line width=\lw,mark=o,mark options={solid}](0,0) -- (5mm,0);}}}   %Símbolo de curva discontinua
\newcommand{\blacksdotted}{\raisebox{2pt}{\tikz{\draw[color=black,dotted,line width=0.75pt,mark=o,mark options={solid}](0,0) -- (5mm,0);}}}   %Símbolo de curva 
\newcommand{\blackdiamond}{\raisebox{1pt}{\tikz{\node[draw,line width=\lww,scale=0.4,diamond,color=my_green,fill=white](){};}}}
\newcommand{\blackcircle}{\raisebox{1pt}{\tikz{\node[draw,line width=\lww,scale=0.5,circle,color=black,fill=white](){};}}}
\newcommand{\ksquare}{\raisebox{1pt}{\tikz{\node[draw,line width=1pt,scale=0.6,rectangle,color=red,fill=white](){};}}}

\newcommand{\pamfour}{orange!70!red}

\pgfplotscreateplotcyclelist{mylist}{
    {red},{blue},{green!50!black},{orange},{blue!50!red},{green!50!blue},{black,densely dotted}
}

\begin{tikzpicture}
    \begin{axis}[
    width=0.98\columnwidth,  %ancho de la figura
    height=2.5in,
    font=\footnotesize,
    xmin=-4, xmax=2,
    ymin=2.4, ymax=2.5,
    xlabel={OMA [dBm]},
    ylabel={MI [bits/channel use]},
    ytick pos=left,
    xtick pos=bottom,
    grid=both,
    grid style = {dashed,lightgray!75},
    legend style = {legend pos=north east, font=\footnotesize, legend cell align=left, row sep=-0.5ex},
    ytick={2.20,2.22,...,2.50},
    xtick={-4,-3,...,2},
    cycle list name=mylist
    ]
    
        
        % SER_ES
        \foreach \col in {5,6,7,8} {
            \addplot+[solid, line width=\lw] table[x index=0,y index=\col] {\datatableSW};
        }

        % \node [draw,font=\footnotesize,fill=white,anchor=north east] at (rel axis cs:0.98, 0.98) {\shortstack[l]{
        %     \blacksolid \hspace{0.01cm} Analytical w/ $r^\star$\\
        %     \blacksdashed \hspace{0.01cm} Analytical w/ $\hat{r}$\\
        %     \hspace{0.08cm} \blackcircle \hspace{0.17cm} Monte Carlo
        % }};
        
    \end{axis}
    
\end{tikzpicture}

